Parallel Matrix Factorization for Binary Response

Predicting user affinity to items is an important problem in applications like content optimization, computational advertising, and many more. While bilinear random effect models (matrix factorization) provide state-of-the-art performance when minimizing RMSE through a Gaussian response model on explicit ratings data, applying it to imbalanced binary response data presents additional challenges that we carefully study in this paper. Data in many applications usually consist of users' implicit response that are often binary -- clicking an item or not; the goal is to predict click rates, which is often combined with other measures to calculate utilities to rank items at runtime of the recommender systems. Because of the implicit nature, such data are usually much larger than explicit rating data and often have an imbalanced distribution with a small fraction of click events, making accurate click rate prediction difficult. In this paper, we address two problems. First, we show previous techniques to estimate bilinear random effect models with binary data are less accurate compared to our new approach based on adaptive rejection sampling, especially for imbalanced response. Second, we develop a parallel bilinear random effect model fitting framework using Map-Reduce paradigm that scales to massive datasets. Our parallel algorithm is based on a "divide and conquer" strategy coupled with an ensemble approach. Through experiments on the benchmark MovieLens data, a small Yahoo! Front Page data set, and a large Yahoo! Front Page data set that contains 8M users and 1B binary observations, we show that careful handling of binary response as well as identifiability issues are needed to achieve good performance for click rate prediction, and that the proposed adaptive rejection sampler and the partitioning as well as ensemble techniques significantly improve model performance.

==> related.tex <==


\section{Related Work}
Our work extends the rich literature on factorization models to provide
a better model fitting strategy with rare binary response that is commonplace
in web applications. We also provide a new model fitting strategy to scale these
methods to massive datasets in a Map-Reduce paradigm. 

Matrix factorization is well known to provide state-of-the-art performance for recommender problems. A
theoretical perspective of this problem was first provided in
\cite{srebro2005}. \cite{koren07,nworkshop} have successfully used this strategy in collaborative filtering applications such as the Netflix challenge. \cite{ruslan:icml08b,ruslan08a} formulate a probabilistic framework using a hierarchical random-effects model where the user and item factors are multivariate
random-effects (factor vectors) that were regularized through zero-mean multivariate
Gaussian priors. These papers used factorization as a tool to solve pure collaborative filtering problems; they do not
work well in applications with significant cold-starts which is commonplace in several applications. 

A desirable
approach would be to have a model that provides predictive accuracy as
matrix factorization for warm-start scenarios but fallbacks on a
feature-based regression model in cold-start scenarios.
Incorporating both warm-start and cold-start scenarios simultaneously in collaborative filtering 
is a well studied problem with a rich literature.  Several methods that
combine content and collaborative filtering have been studied. For instance,
Balabanovic and Shoham~\cite{fab97} present a recommender system that computes user similarities based
on content-based profiles. In \cite{claypool99}, collaborative
filtering and content-based filtering are combined linearly with
weights adjusted based on absolute errors of the
models. In \cite{melville02}, content based models are used to fill up
the rating matrix followed by recommendation based on similarity (memory) based methods \cite{BreeseHK98}. 
In \cite{good99} and \cite{park06}, \textit{filterbots} are used to
improve cold-start recommendations. Schein et al.~\cite{schein03} extend the
aspect model to combine the item content with user ratings under a single
probabilistic framework.  In \cite{agarwal2009regression,matchbox}, a principled solution is proposed by treating user and item factors as random effects and using linear model regression priors on the user and item factors through features. This is generalized in \cite{gmf} so that the regression priors can be non-linear functions which further improves the model predictive accuracy. These solutions based on incorporating features into factorization itself are
superior than the classical methods of dealing with warm-start and cold-start
scenarios simultaneously. 

To scale matrix factorization, stochastic gradient descent
(SGD) is popular \cite{koren2009matrix}. To handle large
data sets using Map-Reduce, Zinkevich et al.~\cite{zinkevich2010parallelized} propose
a parallelized SGD with the simple ``divide and conquer" idea and a
rigorous convergence proof. Gemulla et al.~\cite{gemulla2011large} propose a
parallelized SGD algorithm for matrix factorization that can scale up
to millions of rows and columns. However, these model fitting
algorithms usually consider only the observed response but not
user/item features for ``cold-start" problems. We provide a solution
that can scale factorization methods which use both response and features
in a Map-Reduce framework using a Gibbs sampling approach. 
DeCoste~\cite{decoste} also uses ensemble methods to improve maximum margin matrix factorization methods. However,
the ensembles are trained by initializing the factors at different values, our ensemble approach
is used to partition the data and improve estimates of factors.



==> training.tex <==
\section{Parallelized Model Fitting for Large Data}
\label{sec::parallel}
To scale up the Regression-based Latent Factor Modelling (RLFM) \cite{agarwal2009regression}, we use an ensemble and a divide and conquer approaches. Employing divide-and-conquer, we build ``local" models in subsets of the full data by randomly partitioning it, so that all events of a given user go into the same partition, and run our single machine RLFM implementation on the partitions in parallel.  Employing a novel emsemble approach, the random partitioning and the local modelling is done several times, with parameters of these subsequent training runs initialized from the ones obtained from the first run (details follow), before the output parameters from all the runs in the ensemble are combined to arrive at the final output parameters of the algorithm. There are several runs of random partioning and local model training in the ensemble. The process is delineated in algorithm \ref{algo:rlfmensemble}. The map-reduce algorithm for a single run in the ensemble is mentioned in algorithm \ref{algo:rlfmtraining}. The map-reduce procedure for combining models is given in algorithm \ref{algo:combinemodels}.
 
The RLFM uses an expectation-maximization (EM) procedure to maximize the log-likelihood, as given in Algorithm 1 from Agarwal \emph{et. al.} \cite{Agarwal_Chen_2009}. For quick reference, we provide a simplified view of the same algorithm in algorithm \ref{algo:rlfmsp}. The parameters updated in E-step of the EM algorithm are the user/item specific parameters - the user bias, the item popularity, and the user and item factor estimates. On the other hand, M-step optimizes the (global) regression and variance estimates which are in turn used in the Monte-Carlo E-step to draw out the user/item specific parameters. 

To scale up the computation of M-step parameters, we note partitioning the data to train models on partitions and subsequent averaging of the M-step parameters gives an unbiased estimate of the global M-step parameters. We also observed in practice that across different runs in the ensemble, averaged M-step parameters of all local models within the run, do not yield different results. At the same time, averaging the M-step parameters from multiple runs in the ensemble does not help but adds to complexity and training time. Hence, averaging the M-step parameters from a single run suffices.   

Each run in the ensemble has its partitioning done with a different seed, so the mix of users in partitions across different runs is different. Partitioning function we used to ascertain the different mix of users is explained in algorithm \ref{algo:getpartnum}. In each local model training, the E-step parameters are drawn out from local M-step parameters. As such, we note that simply averaging over the Estep parameters may not be good. Since we now have fixed global M-step parameters obtained above from the first run of the ensemble, we make subsequent runs of the ensemble as ``Estep-only" - we use the global M-step parameters to make single iteration of E-step on the partitions, instead of running the full algorithm \ref{algo:rlfmsp}. We verify that this yeilds more stable and better results and is less resource(grid) utilizaing and shortens the training time significantly.

When running the single machine implementation on partitions in the reducers of the map-reduce framework, for scalability, we also partition user features and the initializing parameters (for runs which require parameters to be initialized from the given set) using the same partitioning function. This way, the training code sees a set of userids in the input data and is delivered the features and the initialization parameters for those same userids, and not all of the userids. This partition of features and parameters are done by algorithm \ref{algo:partitioner}.

The code for the RLFM ensemble, with relevant instructions on how to run it, is documented on the twiki \cite{twiki_code};

\begin{algorithm}
\caption{RLFMSinglePartition}
\emph{MCEM algorithm}
\label{algo:rlfmsp}
\textbf{INPUT:} numIters, doMStep, sampleVector,
input data, user and item features, initParams
\begin{algorithmic}
\IF{$initParams$ are not null}
\STATE Initialize $E$ and $M$ step parameters from $initParams$
\ELSE 
\STATE Initialize all parameters randomly
\ENDIF
\FOR{$iter=1$ to $numIters$}
\STATE \texttt{// Do Monte carlo E-step}
\STATE $numSamples  \leftarrow sampleVector[iter]$
\FOR{$ns=1$ to $numSamples$}
\STATE Draw samples for $u_i$, $\alpha_i$ (user parameters), $v_j$, $\beta_j$ (item parameters)
\ENDFOR
\STATE Average the samples for each type of parameters to obtain output of E-step
\IF{$doMStep==1$}
\STATE \texttt{// Do M-step} 
\STATE Update all the regression parameters($G,D,d0,g0,b$) and variances($A_u, A_v, a_{\alpha}, a_{\beta} $).
\ENDIF
\ENDFOR 
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{PartitionFtrsOrParams}
\label{algo:partitioner}
\textbf{INPUT:} Unshuffled data in form of tuples of type <id><ftr1>..<ftrn>; seed\\
\textbf{OUTPUT:} Shuffled data - partitioned on id and has one part file for each partition
\begin{algorithmic}
\STATE
\STATE \texttt{MAPPER:}
\FOR{each input tuple}
\STATE $partitionNum \leftarrow $ GetPartitionNumber(seed=seed, id = tuple[0])
\STATE Print <$partitionNum$> <tuple>
\ENDFOR
\STATE 
\STATE \texttt{PARTITIONER:} 
\STATE Shuffle mapper output so that each partitionNum maps to one part file 
\STATE 
\STATE \texttt{REDUCER:}
\STATE Remove partitionNum adjoined with the tuple. 
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{GetPartitionNumber}
\label{algo:getpartnum}
\textbf{INPUT:} $id$ (integer), seed(integer$\ge1$), $range$\\
\textbf{OUTPUT:} partitionNumber
\begin{algorithmic}
\STATE Initialize random number generator - setSeed($id$);
\FOR{$i=1$ to $seed$}
\STATE $partNum$=\texttt{rand}() mod $range$;
\ENDFOR
\STATE \textbf{return} $partNum$;
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{CombineModels}
\label{algo:combinemodels}
\textbf{INPUT:} input(=DFS link to local models which are R objects), type(=user or item)\\
\textbf{OUTPUT:} ascii file with <id><params> . 
\begin{algorithmic}
\STATE Create temp files to enforce number of mappers
\STATE
\STATE \texttt{Mapper:}
\STATE Input is a temp file which lists all models assigned to this mapper
\FOR{each model assigned to this mapper}
\STATE Load the model by firing up R
\STATE Extract out and output <id> <params> from the model, depending on whether type=user/item.
\ENDFOR 
\STATE
\STATE \texttt{Reducer:}
\STATE Aggregate the parameters for each id.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{RLFMTraining}
\label{algo:rlfmtraining}
\textbf{INPUT:} seed, doMstep, partitioned initParams, input data(= tuples of form <label><userid><itemid>), partitioned user and item features, number of partitions per run(p), number of factors, number of iterations for the EM (numIters), number of samples to generate in each iteration (sampleVec) ...
\textbf{OUTPUT:} Local models learnt on individual partitions
\begin{algorithmic}
\STATE \texttt{MAPPER:}
\FOR{each input tuple}
\STATE $partitionNum \leftarrow $ GetPartitionNumber(seed=seed, id = tuple[0])
\STATE Print <$partitionNum$> <tuple>
\ENDFOR
\STATE
\STATE \texttt{PARTITIONER:}
\STATE Shuffle mapper output so that each partitionNum maps to one part file
\STATE
\STATE \texttt{REDUCER:}
\STATE Obtain user features from corresponding part-file
\STATE Obtain item features 
\STATE Obtain M-step initializing parameters (could be null)
\STATE Obtain E-step initializing parameters from corresponding part-file (could be null)
\STATE Use all of the above with the input tuple to call RLFMSinglePartition()
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{RLFMEnsemble}
\label{algo:rlfmensemble}
\textbf{INPUT:} input data, user and item features, 
number of runs in ensemble(r, r$\ge 2$), number of partitions per run(p), number of factors,
 number of iterations for the EM (numIters), number of samples to generate in each iteration (sampleVec) ...\\
\textbf{OUTPUT:} E-step parameters (user and item specific parameters), M-step parameters (global regression parameters) 
\begin{algorithmic}
\STATE \texttt{Full RLFM run } 
\STATE set $seed=1$
\STATE Partition user features for $seed$ by calling PartitionFtrsOrParams()
\STATE Set initParams to null 
\STATE Call RLFMTraining() with doMstep=1.
\STATE
\STATE \texttt{Combine Models}
\STATE Load all of the $p$ models one by one on single machine, and average out M-step parameters. These give the final M-step parameters. 
\STATE Call CombineModels(type=user) to obtain user parameters from R objects 
\STATE Call CombineModels(type=item) to obtain item parameters from R objects.  
\STATE 
\STATE \texttt{Estep-only Runs}
\FOR{$seed=2$ to $r$; all runs parallel }
\STATE Partition user features for $seed$ by calling PartitionFtrsOrParams()
\STATE Partition user parameters obtained above after calling CombineModels() by calling PartitionFtrsOrParams() 
\STATE Set initParams to partitioned parameters and averaged Mstep parameters.
\STATE Call RLFMTraining() with doMstep=0, numIters=1, sampleVec set appropriately.
\ENDFOR
\STATE 
\STATE \texttt{Combine Models}
\STATE Mstep parameters already fixed above 
\STATE Call CombineModels(type=user) to obtain final user parameters 
\STATE Call CombineModels(type=item) to obtain final item parameters 
\end{algorithmic}
\end{algorithm}
   

\begin{table}
\caption{The overall AUC for \FEAT, \ARS and \VAR, with different number of factors and ensemble runs.}
\label{table:overallauc}
\vspace{0.1in}
\begin{center}
\begin{tabular}{ccccc}
\hline
Method & Number & 1  & 5  & 10 \\
& of Factors & Ensembled  &Ensembled & Ensembled\\
\hline
MCEM & 3 & 0.6957 & 0.6964 & 0.6964\\
-ARS& 5 & 0.6958 & 0.6964 & 0.6964\\
& 10 & 0.6958 & 0.6964 & 0.6965\\
\hline
MCEM& 3 & 0.6787 & 0.6750 & 0.6742\\
-VAR & 5 & 0.6787 & 0.6750 & 0.6742\\
& 10 & 0.6787 & 0.6750 & 0.6742\\
\hline
FEAT& 3 & 0.6694 & --- & ---\\
-ONLY& 5 & 0.6728 & --- & ---\\
& 10 & 0.6683 & --- & ---\\
\hline
\end{tabular}
\end{center}
\end{table}

